Vision-Language Models in Remote Sensing: Current Progress and Future Trends

The remarkable achievements of ChatGPT and GPT-4 have sparked a wave of interest and research in the field of large language models for Artificial General Intelligence (AGI). These models provide intelligent solutions close to human thinking, enabling us to use general artificial intelligence to solve problems in various applications. However, in remote sensing (RS), the scientific literature on the implementation of AGI remains relatively scant. Existing AI-related research in remote sensing primarily focuses on visual understanding tasks while neglecting the semantic understanding of the objects and their relationships. This is where vision-language models excel, as they enable reasoning about images and their associated textual descriptions, allowing for a deeper understanding of the underlying semantics. Vision-language models can go beyond visual recognition of RS images, model semantic relationships, and generate natural language descriptions of the image. This makes them better suited for tasks requiring visual and textual understanding, such as image captioning, and visual question answering. This paper provides a comprehensive review of the research on vision-language models in remote sensing, summarizing the latest progress, highlighting challenges, and identifying potential research opportunities.

==> TOTO.tex <==
聪聪
1. 摘要和introduction重新总结

3. 添加一个章节, vision language model resources
1) hugging face 
2) LAVIS
3) 

胡媛
1. 表1中除了CNN这种泛指以外的方法，需要加引用；缩写，例如RSIC需要在caption中添加说明
2. 检查文字图标格式
3. 检查引用是否缺失
4. 专业术语统一，例如vision language model和visual language model


1. Fig. 1和Fig. 14重新截图，背景不是纯白，我这边截图背景是灰色的，你们操作一下哈
2. 表1中我把CNN有对应模型的全替换成具体模型了，有的CNN会用到alexnet，vgg，resnet啥的好几个导致表被拉长，一页显示不下了，是否还是改成CNNs然后后面加上这几个具体模型的citation。


Nevertheless, the current version of the topic proposal needs a more detailed description in some critical parts of the proposed paper outline. 

1. Specifically, the authors should provide more details in the application scenarios of the vision-language models to deliver a thorough overview of the actual impact of the missions and the added value they can provide. 
Response: We provide a thorough overview of how vision-language models can be used in the introduction part.

2. Also, the authors could include additional parameters for the estimate of the methods described in Section III such as technology readiness levels and feasibility of the Vision-Language Modelling technologies. 

3. Moreover, they could include a subsection to describe examples of how Vision-Language Models can support and improve research fields of interest for the GRSS community (e.g., object detection, image retrieval), and for the society at large (e.g., the actual implementation of sustainable development goals (SDGs), climate change adaptation and mitigation).
Response: broder impact, espacially for the society at large.


section III除了需要给数量指标，还需要简单总结一下现有方法，有没有什么局限，能怎么改进，简单2-3句话。

Their results also show that text-based semantic relations can significantly improve the few-shot detection performance在描述结果时可以加上类似的描述，说明language在里面的作用


==> table.tex <==

\begin{table*}[ht]
    \centering
    \begin{tabular}{lp{0.5cm}p{1.5cm}p{1cm}p{2cm}p{6cm}}
        \hline
        Method & Year & Task & Visual Encoder & Text Encoder & Datasets \\
        \hline
        fdfd & 2019 & Foundation model &  \\
        Bejiga et al.~\cite{bejiga2019retro} & 2019 & T2IG &  \\
        Chen et al.~\cite{chen2021remote} & 2021 & T2IG &  \\
        Zhao et al.~\cite{zhao2021text} & 2021 & T2IG &  \\
        Xu et al.~\cite{xu2022txt2img} & 2022 & T2IG &  \\
        fdfd & 2019 & T2IR &  \\
        Lobry et al.~\cite{lobry2020rsvqa} & 2020 & VQA & CNN & LSTM & Mutual attention was further designed to enhance the alignment between visual and textual features \\
        Zheng et al.~\cite{zheng2021mutual} & 2021 & VQA & CNN & GRU & introduced a mutual attention network to exploit semantic correspondence between visual and textual features, with a bilinear module to conduct feature fusion \\
        Chappuis et al.~\cite{chappuis2022language} & 2022 & VQA & ResNet-152~\cite{he2016deep} & BERT~\cite{devlin2018bert} & \\
        Al et al.~\cite{al2022open} & 2022 & VQA & Vision Transformer & Transformer & use a transformer decoder that leverages a cross-attention mechanism to integrate the two modalities \\
        Bazi et al.~\cite{bazi2022bi} & 2022 & VQA & Vision Transformer & CLIP~\cite{radford2021learning} & use an attention mechanism to learn correlations between these representations \\
        Yuan et al.~\cite{yuan2022easy} & 2022 & VQA & CNN &  RNN & cross-modal attention for fusion \\ 
        Yuan et al.~\cite{yuan2022change} & 2022 & VQA & ViT~\cite{} & RNN & feature concatenation \\
        Li et al.~\cite{li2017zero} & 2017 & Zero-shot Scene Classification & GoogLeNet~\cite{simonyan2014very} & Word2vec~\cite{mikolov2013efficient} & construct a semantic graph to capture inter-class relationship. \\
        Sumbul et al.~\cite{sumbul2017fine} & 2017 & Zero-shot Scene Classification & CNN & Word2vec~\cite{mikolov2013efficient} &  trained a compatibility function to establish the association between image features and semantic embeddings \\
        Quan et al.~\cite{quan2018structural} & 2018 & Zero-shot Scene Classification & GoogLeNet~\cite{simonyan2014very} & Word2vec~\cite{mikolov2013efficient}  & use a Sammon embedding algorithm to modify semantic space prototypes to have a more consistent class structure with visual space prototypes.\\
        Wang et al.~\cite{wang2021distance} & 2021 & Zero-shot Scene Classification & ResNet-152~\cite{he2016deep} & Word2vec~\cite{mikolov2013efficient}  & propose a distance-constrained semantic autoencoder to align the visual features and semantic representations \\
        Li et al.~\cite{li2022generative} & 2022 & Zero-shot Scene Classification & ResNet-101~\cite{he2016deep} & Word2vec~\cite{wang2016relational}, Fasttest~\cite{joulin2016bag,bojanowski2017enriching}, Glove~\cite{xian2016latent}, and BERT~\cite{devlin2018bert} & a generator network was trained to synthesize image features from class semantics \\
        Zhang et al.~\cite{zhang2023text} & 2023 & Few shot Detection & Faster RCNN & Glove~\cite{xian2016latent} & text semantic fusion relation graph reasoning \\
        Lu et al.~\cite{lu2023few} & 2023 & Few shot Detection & Faster RCNN & GRU~\cite{cho2014learning} & propose a cross-modal assembly module to integrate text-modal knowledge into RoI visual-modal features effectively and comprehensively \\
        fdfd & 2019 & Few-shot Semantic Segmentation &  \\
        fdfd & 2019 & Multimodal data analysis &  \\
        \hline
    \end{tabular}
    \caption{Summary of vision-language models in remote sensing.}
    \label{tab_summary}
\end{table*}

